Transformer-based Variable-rate Image Compression with Region-of-interest Control

This paper proposes a transformer-based learned image compression system. It is capable of achieving variable-rate compression with a single model while supporting the region-of-interest (ROI) functionality. Inspired by prompt tuning, we introduce prompt generation networks to condition the transformer-based autoencoder of compression. Our prompt generation networks generate content-adaptive tokens according to the input image, an ROI mask, and a rate parameter. The separation of the ROI mask and the rate parameter allows an intuitive way to achieve variable-rate and ROI coding simultaneously. Extensive experiments validate the effectiveness of our proposed method and confirm its superiority over the other competing methods.

==> Tables/complexity.tex <==
\begin{table}
\caption{Comparison of computational complexity}
\centering
\begin{tabular}{|c||c|c|}
\hline
              & kMACs/px & Params (M) \\ \hline
\texttt{Base}              & 718.5    & 17.66  \\ \hline
\texttt{CNN+SFT}           & 1480.16  & 27.56  \\ \hline
ICCV'21 (on \texttt{Base}) & 1915.8   & 21.71  \\ \hline
Ours              & 1070.68  & 32.7   \\ \hline
\end{tabular}
\label{tab:complexity}
\end{table}
